Evaluation of Differentially Constrained Motion Models for Graph-Based Trajectory Prediction

Given their flexibility and encouraging performance, deep-learning models are becoming standard for motion prediction in autonomous driving. However, with great flexibility comes a lack of interpretability and possible violations of physical constraints. Accompanying these data-driven methods with differentially-constrained motion models to provide physically feasible trajectories is a promising future direction. The foundation for this work is a previously introduced graph-neural-network-based model, MTP-GO. The neural network learns to compute the inputs to an underlying motion model to provide physically feasible trajectories. This research investigates the performance of various motion models in combination with numerical solvers for the prediction task. The study shows that simpler models, such as low-order integrator models, are preferred over more complex, e.g., kinematic models, to achieve accurate predictions. Further, the numerical solver can have a substantial impact on performance, advising against commonly used first-order methods like Euler forward. Instead, a second-order method like Heun's can greatly improve predictions.

==> method.tex <==
\section{Proposed Method}
\label{sec:proposed_method}

\subsection{Data set}
\label{sec:dataset}
For training and testing we use three different data sets: \highd\cite{highDdataset}, \round\cite{rounDdataset}, and \ind\cite{inDdataset}.
The data sets contain recorded trajectories from different locations in Germany, including various highways, roundabouts and intersections.
The data was captured at 25 Hz, and contain several hours of naturalistic driving data of considerable quality, much in response to previously available data sets, such as the widely cited NGSIM---known to suffer from several problems affecting the overall quality \cite{coifman2017critical}.


\subsubsection{Preprocessing}
Data extraction follow an ego-centric approach, meaning we build the input graph around a particular vehicle, see \Cref{fig:ego_graph}.
The number of nodes in the graph may change over the observation window (added or removed during the recording stage), meaning the sequence of feature history pertaining to nodes could be of different length.
Observations for training and inference cover at most 3~s, and at least one sample.
Regardless, we require that the model should output a prediction for all nodes in the graph over a 5~s long horizon, despite possible information scarcity.
We argue that this is most general approach, with connection to real applications where it is unlikely to wait in order to infer a prediction.
During the preprocessing stage, the input and target data is down-sampled by a factor of 5, effectively setting the sampling time $d_t=0.2$~s.

\begin{figure}[!t]
	\centering
	\includegraphics[width=\columnwidth]{img/ego-graph-temp}
	\caption{Graph construction for a highway forecasting problem. The graph is centered around a randomly selected vehicle.}
	\label{fig:ego_graph}
\end{figure}

\subsection{Input Features}
\label{sec:input_features}
The used data sets offer a collection of traffic agent trajectories and structural information from recorded traffic data.
We shall here distinguish between \emph{node}, \emph{context} and \emph{static} features.
Both node and context features are time-varying by nature, typically referring to positional information, but are separated here since the context features depend on the given data set. 
In contrast, static features refers to time-invariant information, e.g agent dimensions.
We denote the union of available features as the set of observations $\mathbb{X}$.

\subsubsection{Node Features}
\label{sec:node_features}
The time-varying features pertaining to the nodes are summarized in \Cref{tab:node_feat}.
These include planar positions, velocities and accelerations over the observation window. 
The planar coordinates are given relative to a pre-defined origin $(x_0, y_0)$, that is dependent on the current data set.
In the case for \highd, this refers to the graph-centered node's initial position at the recording instance.
For \round\ and \ind, these refer to the roundabout circumcenter, and the road junction point of intersection, respectively.

\begin{table}[!h]
	\vspace{-0.1in}
	\caption{Node features}
	\label{tab:node_feat}
	\centering
	\begin{tabular}{c l l}
		\toprule
		Feature & Description & Unit\\
		\midrule
		$x$ & Longitudinal coordinate with respect to $x_0$ & m\\ 
		$y$ & Lateral coordinate with respect to $y_0$ & m\\ 
		$v_x$ & Instantaneous longitudinal velocity & m/s \\
		$v_y$ & Instantaneous lateral velocity & m/s\\
		$a_x$ & Instantaneous longitudinal acceleration & m/$\text{s}^2$ \\
		$a_y$ & Instantaneous lateral acceleration & m/$\text{s}^2$\\
		$\psi$ & Yaw angle  & rad \\
		\bottomrule
	\end{tabular}
\end{table}

\subsubsection{Road Context Features}
We adopt the methods presented in our previous work \cite{westny2021vehicle}, meaning that for \highd, these context features adds additional information on lateral position with respect to the current lane centerline and the overall road center, respectively (see \Cref{tab:highd_context}).
The first of the two, denoted $d_l$, refers to the vehicle's lateral deviation from the current lane center; bounded to the interval $[-1, 1]$ according to 
\begin{equation}
    d_l = 2\frac{y_l - l_{y,l}}{l_w}-1,
\end{equation}
where $y_l \triangleq y+y_0$ refers to the local coordinate of the vehicle in the recorded data frame, $l_{y,l}$ is the lateral coordinate of the left lane divider for the current lane, and $l_w$ as the lane width.
The second feature, $d_r$, has an equivalent definition, replacing the lane width with the breadth of the road as well as using the left-most lane divider as reference.
The addition of these features are motivated by their expressiveness in lane-changing situations as well as their adaptability toward road geometry \cite{westny2021vehicle}.

For \round\ and \ind, the context features are defined as polar coordinates with respect to the origin $(x_0, y_0)$, previously defined in \cref{sec:node_features}; summarized in \Cref{tab:round_context} and calculated according to:
\begin{subequations}
	\begin{align}
		r = \sqrt{(x_0 - x)^2 + (y_0 - y)^2}\\
		\theta = \text{atan2}(y_0 - y, x-x_0)
	\end{align}
\end{subequations}
where $x$ and $y$ are the node planar coordinates.

\begin{table}[!h]
	\vspace{-0.1in}
	\caption{HighD road context features} 
	\label{tab:highd_context}
	\centering
	\begin{tabular}{c l l}
		\toprule
		Feature & Description & Unit\\
		\midrule
		$d_y$ & Lateral deviation from the current lane centerline & -\\
		$d_r$ & Lateral deviation from the road center & -\\
		\bottomrule
	\end{tabular}
\end{table}

\begin{table}[!h]
	\vspace{-0.1in}
	\caption{RounD \& InD road context features} 
	\label{tab:round_context}
	\centering
	\begin{tabular}{c l l}
		\toprule
		Feature & Description & Unit\\
		\midrule
		$r$ & Euclidean distance from the origin & m\\
		$\theta$ & Angle relative to the origin & rad\\
		\bottomrule
	\end{tabular}
\end{table}

\subsubsection{Static Features}
Lorem ipsum...

\begin{table}[!h]
	\vspace{-0.1in}
	\caption{Static features}
	\label{tab:struc_feat}
	\centering
	\begin{tabular}{c l l}
		\toprule
		Feature & Description & One-hot encoding\\
		\midrule
		$\mathcal{C}$ & Vehicle class & M = $[1,0,0]$, A = $[0,1,0]$, T = $[0,0,1]$\\ 
		\bottomrule
	\end{tabular}
\end{table}


\subsection{Model Architecture}
Add model architecture here. 

\subsubsection{Temporal Graph Neural Network}
[ADD WORKSHOP PROPOSAL]

\begin{subequations}
\begin{align}
	r_t &= \sigma(W_{xr}x_t + b_{xr} + W_{hr}h_{t-1} + b_{hr}) \\
	z_t &= \sigma(W_{xz}x_t + b_{xz} + W_{hz}h_{t-1} + b_{hz}) \\
	n_t &= \text{tanh}(W_{xn}x_t + b_{xn} + r_t \odot(W_{hn}h_{t-1} + b_{hn})) \\
	h_t &= (1 - z_t) \odot n_t + z_t \odot h_{t-1}
\end{align}
\end{subequations}

\subsubsection{Motion Model}
\label{sec:motion_model}
There exists well-established methods for modeling systems in target tracking \cite{li2003survey} and predictive control applications \cite{paden2016survey} that could be adopted for behavior prediction.
However, while for example wheeled vehicles are approximately described using nonholonomic constrained models such as the widely used kinematic single-track model---similar formulations require knowing the length of the wheelbase which could be difficult to estimate online.
More importantly, other traffic agent types, such as pedestrians, may not share the same differential constraints.
The commonality between the agents however, is that one typically formulate the equations of motion mathematically using (ordinary) differential equations.
With the recent breakthrough of neural differential equations \cite{chen2018neuralode}, we argue that such a flexible formulation could apply here by instead learning the underlying motion model but still enjoying the benefits of smooth trajectories.

Consider a sequential forecasting model $f$.
In conventional black-box estimation (by e.g. recurrent neural networks), the model parameters $\bm{\theta}$ are learned by minimizing the $n$-step prediction error between a discrete target and a directly predicted output $\bm{x}_{k}$
\begin{equation}
	\bm{x}_{k} = f(\bm{x}_{k-1}, \bm{\theta})
\end{equation}
In contrast, a neural ODE should learn to output the state derivative
\begin{equation}
	\frac{d\bm{x}(t)}{dt} = f(\bm{x}(t), \bm{\theta})
\end{equation}
where the states can be retrieved using standard tools for numerical integration \cite{ascher1998computer}.
The benefit of such a parameterization is that we can generate smooth trajectories without expert-knowledge, and instead have the network learn the model structure.
We denote this part of the network as the \emph{motion model} $f$ and model it as a multi-layered perceptron with ELU activation functions.
The function $f$ accepts two input vectors: the prior state $\bm{x}$ and the current input $\bm{u}$.
We use a \emph{grey box} approach for the design of $f$, meaning we construct the motion model in a partially informed manner.
For example, in the simplest case where we have two model states $(x, y)$, we employ two separate ODEs $f_1$ and $f_2$ (solved in parallel) with their respective inputs such that
\begin{subequations}
	\begin{align}
		\dot{x} &= f_1(x, y, u_1) \\
		\dot{y} &= f_2(x, y, u_2)
	\end{align}
\end{subequations}
The same design-principles is employed to higher-order models, letting the neural ODE model the highest order state-transition equations.
\begin{subequations}
	\begin{align}
		\dot{x} &= v_x \\
		\dot{y} &= v_y \\
		\dot{v}_x &= f_1(v_x, v_y, u_1) \\
		\dot{v}_y &= f_2(v_x, v_y, u_2)
	\end{align}
\end{subequations}
Importantly, we fix the number of motion models inputs to two, motivated by the degrees of freedom in ground vehicles.

\subsubsection{Probabilistic Output}
\label{sec:probabilistic_output}
To produce multi-modal future predictions, the network structure is inspired by mixture density networks \cite{bishop2006pattern}.
Each output vector $\bm{y}_k$ of the complete model contain \emph{mixing coefficients} $\bm{\pi}^j$, along with mean $\bm{\mu}_k$ of the states $\bm{x}_k$ and the distribution covariance $\bm{\Sigma}_k$.
\begin{equation}
	\bm{y}_k = \left( \bm{\pi}^j, \big\{\bm{\mu}_k^j,  \bm{\Sigma}_k^j\big\}_{j=1}^{M} \right) 
\end{equation}
For a symmetric and positive definite covariance matrix $\bm{\Sigma}$, the multivariate Gaussian distribution is written as
\begin{equation}
	\mathcal{N}(\bm{x} | \bm{\mu}, \bm{\Sigma}) = \frac{\exp\left[-\frac{1}{2} (\bm{x} - \bm{\mu})^\text{T} \bm{\Sigma}^{-1} (\bm{x} - \bm{\mu})\right]}{\sqrt{(2\pi)^n |\bm{\Sigma}|}}
\end{equation}
where $\bm{x}$ is a real $n$-dimensional column vector.
The distribution is used to formulate the learning task, here $\bm{\mu}$ and $\bm{\Sigma}$ may represent the learnable distribution mean and covariance.
The probability density $\text{Pr}(\bm{x}_{k+1} | \bm{y}_k)$ of the next state $\bm{x}_{k+1}$ (target vector) given the output vector $\bm{y}_k$ is defined as follows:
\begin{equation}
	\text{Pr}(\bm{x}_{k+1} | \bm{y}_k) = \sum_{j=1}^M \bm{\pi}^j \phi(\bm{x}_{k+1} | \bm{\mu}_k^j, \bm{\Sigma}_k^j)
\end{equation}
where $\phi$ is a Gaussian kernel of the form
\begin{equation}
	\label{eq:gaussian-kernel}
	\phi(\bm{x}_{k+1} | \bm{\mu}_k, \bm{\Sigma}_k) = \frac{\exp\left[-\frac{1}{2} (\bm{x}_{k+1}  - \bm{\mu}_k)^\text{T} \bm{\Sigma}^{-1}_k (\bm{x}_{k+1}  - \bm{\mu}_k)\right]}{\sqrt{(2\pi)^n |\bm{\Sigma}_k|}}
\end{equation}
To determine the sequence loss, we formulate the objective as the negative-log likelihood
\begin{equation}
	\label{eq:seq_loss}
	\mathcal{L}_{NLL}(\mathbf{x}) =\sum_{k=1}^T -\log \left(\sum_j \bm{\pi}^j\phi(\bm{x}_{k+1} | \bm{y}_k)\right)
\end{equation}
where $T$ denotes the final sample of the full prediction horizon.
Note that the mini-batch dimension is omitted here for brevity.

\subsubsection{Uncertainty Propagation}
Combining probabilistic outputs together with sequence generation tasks has been investigated to a large degree \cite{graves2013generating, zyner2019naturalistic, messaoud2020attention, deo2018convolutional}.
However, a problem we identified with some of these works is that while the \emph{a priori} state estimates are conditioned on previous outputs, the predicted covariance is not.
This is because they have the model directly output the covariance matrix at very prediction step.
For multi-step forecasting, it is reasonable that the current uncertainty should depend on prior predictions, and to provide such an estimate we propose the use of an \emph{Extended Kalman filter} (EKF) prediction step for every output.
For a given a differentiable state-transition function $f$, input $\bm{u}_k$ and process noise $\bm{w}_k$:
\begin{equation}
	\label{eq:state_transition}
	\bm{x}_{k+1} = f(\bm{x}_k, \bm{u}_k) + \bm{w}_k,
\end{equation}
the prediction step of the EKF is written as:
\begin{subequations}
	\begin{align}
		\hat{\bm{x}}_{k+1} &= 	f(\hat{\bm{x}}_{k|k}, \bm{u}_k) \\
		\bm{P}_{k+1} &= \bm{F}_k \bm{P}_{k|k} \bm{F}_k^{\text{T}} + \bm{G}_k\bm{Q}_k\bm{G}_k^{T}
	\end{align}
\end{subequations}
where
\begin{equation}
	\bm{F}_k = \frac{\partial f}{\partial \bm{x}}\Bigr|_{\hat{\bm{x}}_{k|k}, \bm{u}_k}
\end{equation}
In the equations above, $\hat{\bm{x}}$ and $\bm{P}$ refer to the state estimate and state covariance estimate, respectively.
The matrix $\bm{Q}_k$ denotes the \emph{process noise} and should in combination with $\bm{G}_k$ describe uncertainties in the state-transition function e.g. due to noisy inputs or modeling errors.
The EKF formulation fits well into the overall modeling framework with $f$ as the motion model, $\bm{u}$ as its input produced by the decoder network and the state estimates $\hat{\bm{x}}$ taken as $\bm{\mu}$ in the Gaussian kernel function.

The interesting challenge with this addition to the model is how to implement the state covariance matrix $\bm{P}$ and its respective process noise. 
The solution we found, contrasting several previous works on this topic is that instead of having the network produce the full covariance matrix of the distribution, it should learn to produce the covariance $\bm{Q}_k$ for every time step $k$.
We assume that the process noise $\bm{w}$ enters into the two highest-order states, where $\bm{w}$ has zero-mean and covariance matrix $\bm{Q}$ according to
\begin{equation}
	\bm{Q} = \begin{pmatrix}
		\sigma_{1}^2 & \rho \sigma_{1} \sigma_{1} \\ 
		\rho \sigma_{1} \sigma_{2} & \sigma_{2}^2
	\end{pmatrix}
\end{equation}
where $\rho$ is the correlation between the above-mention states and $\sigma_{1} > 0, \sigma_{2} > 0$.
To get the correct signs of the standard deviations and correlation coefficient, they are commonly passed through an exponential function and hyperbolic tangent \cite{bishop2006pattern, graves2013generating, zyner2019naturalistic, deo2018convolutional, hu2018probabilistic}.
We instead opted for SoftPlus and SoftMin activations for added numerical stability.

How to construct $\bm{G}_k$ depend on the assumptions about the noise $\bm{w}_k$ and how it enters into $f$. 
If it is assumed to be non-additive, such that $\bm{x}_{k+1} = f(\bm{x}_k, \bm{u}_k, \bm{w}_k)\neq$ \cref{eq:state_transition}, then $\bm{G}_k$ is defined by the Jacobian:
\begin{equation}
	\bm{G}_k = \frac{\partial f}{\partial \bm{w}}\Bigr|_{\hat{\bm{x}}_{k|k}, \bm{u}_k}
\end{equation}
While this assumption is often a design-choice, such a formulation is necessary if we would employ a completely general neural ODE motion model, where e.g. each input enters into every predicted state.
By the grey box approach and assuming the noise is additive, we are free to design $\bm{G}_k$ as a matrix of constants.
For the case where we have two states $(x, y)$, we have that $\bm{G}_k = d_t \cdot I_{2}$, where $d_t$ is the sample time.
For higher order state-space models, one can generalize $\bm{G}_k$: 
\begin{equation}
	\bm{G}_k =  d_t 
	\begin{pmatrix}
		 0 & 0 \\ 
		 \vdots & \vdots \\ 
		 1 & 0 \\ 
		 0 & 1
	\end{pmatrix}
\end{equation}

In conclusion, the encoder-decoder network should learn to produce the input to the motion model $\bm{u}_k$ and covariance $\bm{Q}_k$ that minimize the loss function previously presented in \cref{eq:seq_loss} such that:
\begin{equation}
	\bm{\mu}_k \coloneqq f(\hat{\bm{x}}_k, \bm{u}_k), \quad \bm{\Sigma}_k \coloneqq \bm{P}_k
\end{equation}
An interesting consequence is that this formulation simplifies the task of generating $\bm{\Sigma}_k$ when the number of states $>2$. 
In all considered previous works, the authors only considered the Bi-variate Gaussian case in which the covariance matrix may be constructed to be positive definite using simple constraints on the network outputs \cite{graves2013generating, zyner2019naturalistic, messaoud2020attention, deo2018convolutional, makansi2019overcoming}.
By our approach, the method can be generalized to any number of states as long as $\bm{F}_k$ and $\bm{G}_k\bm{Q}_k\bm{G}_k^{T}$ adhere to conventional design rules.
\subsubsection{Winner Takes All}
Mixture density network are notoriously difficult to train---often attributed to numerical instabilities in higher dimensions.
To alleviate some of these problems, one typically trains the network in sequence by first learning the mean and then learning the variance. 
Although this might lead to increased stability in the training process, many MDNs still suffer from mode collapse. 
These problems were investigated in detail by Maksani \etal in \cite{makansi2019overcoming}.
To that end, we adopt their proposed method, \emph{Evolving Winner Takes All} loss and apply it during the first training epochs:
\begin{subequations}
	\begin{align}
		\mathcal{L}_{WTA} &= \sum_{j=1}^K w_j \ell(\bm{\mu}_k^j, \bm{x}_{k+1}) \\
		w_i &= \delta (i = \argmin_j \ell(\bm{\mu}_k^j, \bm{x}_{k+1}))
	\end{align}
\end{subequations}
where $K$ represent the current maximum number of winners (epoch dependent) and $\delta(\cdot)$ is the Kronecker delta, returning 1 when the condition is true, else 0. 
For fast initial convergence, we chose $\ell(\cdot)$ to be the \emph{Huber} loss function, used for winner selection and training.
As mentioned, the top $K$ winners change over time, initially using the upper number of mixtures $M$ and gradually decreasing toward 1 as training progresses before switching objective. 



